Long-term, orbital, and rapid variations of the Be star V923 Aql = HD 183656

We present the latest results of a long-term observational project aimed at observing, collecting from the literature, and homogenising the light, colour, and spectral variations of the well-known emission-line Be star V923 Aql. Our analysis of these parameters confirms that all of the observables exhibit cyclic changes with variable cycle length between about 1800 and 3000 days, so far documented for seven consecutive cycles. We show that these variations can be qualitatively understood within the framework of the model of one-armed oscillation of the circumstellar disk, with a wave of increased density and prograde revolution in space. We confirm the binary nature of the object with a 214.716 day period and estimate the probable system properties. We also confirm the presence of rapid light, and likely also spectral changes. However, we cannot provide any firm conclusions regarding their nature. A quantitative modelling study of long-term changes is planned as a follow-up to this work.

==> abstract <==

\title{Long-term, orbital, and rapid variations \\ 
of the Be star V923 Aql = HD~183656
\author{M. Wolf~\inst{1}\and
P. Harmanec\inst{1}\and
H.~Bo\v{z}i\'c~\inst{2}\and
P.~Koubsk\'y~\inst{3}\and
S.~Yang\inst{4}\and
D.~Ru\v{z}djak\inst{2}\and
M.~\v{S}lechta\inst{3}\and \\
H.~Ak\inst{5}\and
H.~Bak\i\c{s}~\inst{6}\and
V.~Bak\i\c{s}~\inst{6}\and
A.~Opli\v{s}tilov\'a~\inst{1}\and
K.~Vitovsk\'y~\inst{1}
                    }

We present the latest results of a long-term observational project
aimed at observing, collecting from the literature, and homogenising
the light, colour, and spectral variations of the well-known 
emission-line Be star V923 Aql. Our analysis
of these parameters confirms that all of the observables exhibit
cyclic changes with variable cycle length between about 1800 and 3000
days, so far documented for seven consecutive cycles. We show that these
variations can be qualitatively understood within the framework of
the model of one-armed oscillation of
the circumstellar disk, with a wave of
increased density and prograde revolution in space. We confirm
the binary nature of the object with
a 214.716 day period and estimate the
probable system properties. We also confirm the presence of rapid light,
and likely also spectral changes. However, we cannot provide any firm 
conclusions regarding their nature.
A quantitative modelling study of long-term
changes is planned as a follow-up to this work.

\keywords{binaries: spectroscopic --
  stars: emission-line, Be --
  stars: early-type --
  stars: individual: V923 Aql  --
  stars: fundamental parameters }

